Dynamics of Majority Rule on Hypergraphs

A broad range of dynamical systems involve multi-body interactions, or group interactions, which may not be encoded in traditional graphical structures. In this work, we focus on a canonical example from opinion dynamics, the Majority Rule, and investigate the possibility to represent and analyse the system by means of hypergraphs. We explore the formation of consensus and restrict our attention to interaction groups of size $3$, in order to simplify our analysis from a combinatorial perspective. We propose different types of hypergraph models, incorporating modular structure or degree heterogeneity, and recast the dynamics in terms of Fokker-Planck equations, which allows us to predict the transient dynamics toward consensus. Numerical simulations show a very good agreement between the stochastic dynamics and theoretical predictions for large population sizes.

==> SpatialMR.tex <==
\chapter{Spatial Majority Rule Dynamics}\label{spatialMR}
\section{Spin Dynamics}
In this Chapter we shall consider MR dynamics on regular lattice structures. Up until to this point, we have considered hypergraph topologies for which the concept of space was not well defined. However, when it comes to modelling opinion dynamics on physical structures, spatial effects become important. The study of opinion dynamics in spatial contexts is frequently referred to as \textit{spin dynamics} \cite[Chapter 8]{krapivsky2010kinetic}. This name originated in the statistical physics literature, where \textit{spins} refer to magnetic dipole alignments in ferromagnetic materials. The Ising-Glauber (IG) model \cite{glauber1963time} is perhaps the most famous model in this context. Each lattice site is occupied by a spin which can be in one of two states, generally denoted by the values $\pm1$. In the VM and IG models, spins are assumed to interact only with their nearest neighbours on adjacent lattice sites. In the MR model, hyperedges encompass contiguous groups of nodes on the lattice. These restrictions give rise to spatial correlations between spins occupying different lattice sites. \newline

\begin{figure}
    \begin{minipage}{0.2\linewidth}
        \centering
        \includegraphics[height=4cm,width=\linewidth]{30META0.eps}
    \end{minipage}\hfill
    \begin{minipage}{0.2\linewidth}
        \centering
        \includegraphics[height=4cm,width=\linewidth]{30META20.eps}
    \end{minipage}\hfill
    \begin{minipage}{0.2\linewidth}
        \centering
        \includegraphics[height=4cm,width=\linewidth]{30META200.eps}
    \end{minipage}\hfill
    \begin{minipage}{0.2\linewidth}
        \centering
        \includegraphics[height=4cm,width=\linewidth]{30META220.eps}
    \end{minipage}\hfill
    \begin{minipage}{0.2\linewidth}
        \centering
        \includegraphics[height=4cm,width=\linewidth]{30META270.eps}
    \end{minipage}\hfill
    \caption[Metastable state formation on a square lattice]{Snapshots of a $30^{2}$ square lattice at $t=0,20,200,220$ and $270$ showing the formation of a stripe-like metastable state (produced using the ``imagesc'' function in MATLAB).}
    \label{squaremeta}
\end{figure} 

\noindent With regard to MR dynamics on regular lattice structures, a number of studies have been published in which significant progress has been made.
Mobilia and Redner \cite{mobilia2003majority} considered a generalised version of the Majority Rule known as the Majority-Minority (MM) Model, in which all spins in the interaction group adopt the majority opinion with probability $q\in\left[0,1\right]$ and the minority opinion with probability $1-q$. It follows that when $q=1$, MM dynamics reduce to MR dynamics. This study shall be the main focus of Section \ref{ring}.\newline

\noindent Further progress was made from a numerical perspective by Chen and Redner \cite{chen2005majority} who investigated MR dynamics on $2,3$ and $4$-dimensional hypercubic lattices. The authors found the critical dimension to be greater than $4$, where the critical dimension is defined as being the spatial dimension above which mean field theory becomes valid \cite{cardy1996scaling}. The authors also reported the emergence of long-lived metastable states arising from the formation of clusters of spins in opposite orientations, which were observed to appear approximately $33\%$ of the time in two dimensions and $8\%$ of the time in three dimensions. The coherent geometry of these long-lived states is intriguing. In two dimensions, the metastable states take the form of stripes spanning the square lattice. In three dimensions, these coherent states take the form of slabs. Figure \ref{squaremeta} gives a sample of such simulation results on a square lattice of $30^{2}$ spins, where the emergence of a stripe-like metastable state is apparent. Time is measured in units of Monte Carlo steps per spin. In order to generate these figures, a lattice was constructed in MATLAB whereby at time $t=0$, each spin was assigned the value $1$ or $-1$ at random. At each iteration, a spin was chosen uniformly at random from the lattice and two of its nearest neighbours were randomly chosen to form the interaction group of size $3$. As usual, all spins in the group adopted the majority opinion. Periodic boundary conditions were imposed on the lattice, hence the dynamics were effectively evolving on the surface of a torus. This update process was repeated until consensus was eventually reached in the system. \newline

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth,height=8cm]{P30SquareTIMEnogrid.eps}
    \caption[Consensus time distribution on a square lattice]{Consensus time distribution for MR dynamics on a $30^{2}$ square lattice, produced with $10^{4}$ realisations of the stochastic dynamics.}
    \label{ConsensusTimeDistributions}
\end{figure}

\noindent The formation of such long-lived metastable states has profound implications for the associated consensus time distribution, which we shall denote by $P_{N}\left(t\right)$. Figure \ref{ConsensusTimeDistributions} illustrates a two-time scale approach to consensus on the two-dimensional square lattice. The first time scale is relatively short and reflects the fact that the system reaches consensus without collapsing into a metastable state most of the time. The second time scale is much longer, and is attributed to the formation of the aforementioned metastable configurations which take a relatively long time to break down. This is reflected by the noisy asymptotic tail of the distribution. The metastable state on the $30^{2}$ lattice in Figure \ref{squaremeta} was observed to disappear after $650$ time steps. This lies well within the asymptotic tail of the associated consensus time distribution given in Figure \ref{ConsensusTimeDistributions}. Similar behaviour is observed in the IG model whereby the two-dimensional square lattice is partitioned into perfectly straight stripes of opposing magnetisation \cite{blanchard2013frozen,gleiser2002metastable}. However in this instance the stripe states last indefinitely, thereby preventing the system from reaching uniform consensus. In this way, spatial MR dynamics give rise to highly sophisticated behaviour that is largely analytically intractable. For this reason we will focus our efforts on the one-dimensional case for the remainder of this Chapter.

\section{Exit Probability on a Ring}\label{ring}
\noindent In this Section we shall approximate the exit probability of a one-dimensional system of spins evolving in accordance with MR dynamics. We follows the workings of Mobilia and Redner \cite{mobilia2003majority} closely, though ultimately arrive at a different result. Let us consider a line of $N$ spins, each of which can be in the $+1$ state or the $-1$ state. Each spin has two nearest neighbours, and we restrict our attention to interacting triangles. For the purpose of our computational analysis we impose periodic boundary conditions at each end of the line, so that in effect we are considering a ring of spins. The system evolves as follows at each time step:
\begin{enumerate}
    \item Choose a spin uniformly at random from the ring. Let us denote this spin by $S_{j}$, where the subscript $j\in\{1,...,N\}$ indicates the position of the spin on the ring.
    \item Spins $S_{j-1},S_{j}$ and $S_{j+1}$ form the triangle (the hyperedge).
    \item All $3$ spins adopt the majority opinion of the group.
\end{enumerate}
 This process is repeated \textit{ad infinitum} or until consensus is necessarily reached on a finite ring. Note that spin $S_{j}$ can belong to three distinct interacting triangles: $\{S_{j-2},S_{j-1},S_{j}\}, \{S_{j-1},S_{j},S_{j+1}\}$ and $\{S_{j},S_{j+1},S_{j+2}\}$. Consider a group of three contiguous spins, denoted by $S,S'$ and $S''$. The rate $W$ at which spin $S$ flips in accordance with MR dynamics is encoded in the \textit{rate equation}
\begin{equation}\label{MRRateEq}
    W\left(S\rightarrow -S\right) = 1+S'S''-S\left(S'+S''\right).
\end{equation}
Equation (\ref{MRRateEq}) reflects the fact that spin $S$ will only flip if it is strictly in the minority. Given that $S_{j}$ can belong to three distinct triangles, the rate at which spin $S_{j}$ flips is given by
\begin{align}
    W\left(S_{j}\rightarrow -S_{j}\right) &= 3 + S_{j-2}S_{j-1} + S_{j-1}S_{j+1} + S_{j+1}S_{j+2} \nonumber \\ &-S_{j}\left(2S_{j-1}+2S_{j+1}+S_{j-2}+S_{j+2}\right).
\end{align}
Let $P\left(\{S\},t\right)$ be the probability that the system is in configuration $\{S\}$ at time $t$. The the evolution of the probability density function is governed by the master equation
\begin{equation}\label{MRProbMaster}
    \frac{d}{dt}P\left(\{S\},t\right) = \sum_{k}\left[W\left(-S_{k}\rightarrow S_{k}\right)P\left(\{S\}_{k},t\right) - W\left(S_{k}\rightarrow-S_{k}\right)P\left(\{S\},t\right)\right]
\end{equation}
where the summation index $k$ runs over all lattice sites and $\{S\}_{k}$ is the same configuration as $\{S\}$ with the exception of the spin at site $k$, which is flipped. The gain term on the right hand side of equation (\ref{MRProbMaster}) accounts for transitions into configuration $\{S\}$ from $\{S\}_{k}$ following the flipping of the spin at site $k$. Similarly, the loss term on the right hand side of equation (\ref{MRProbMaster}) accounts for transitions out of configuration $\{S\}$ resulting from the flipping of the spin at lattice site $k$.\newline

\noindent Let $\left<S_{j}\left(t\right)\right>$ denote the average state of the spin at lattice site $j$, where angular brackets indicate an average taken over all possible configurations of the system. This is referred to as the \textit{magnetisation}. Using the fact that $\left<S_{j}\right> = \sum_{\{S\}}S_{j}P\left(\{S\},t\right)$, we can calculate its evolution as follows:
\begin{align}
    &\frac{d}{dt}\left<S_{j}\right> = \sum_{\{S\}}S_{j}\frac{d}{dt}P\left(\{S\},t\right) \nonumber \\
    &= \sum_{\{S\}}S_{j}\sum_{k}\left[W\left(-S_{k}\rightarrow S_{k}\right)P\left(\{S\}_{k},t\right) - W\left(S_{k}\rightarrow-S_{k}\right)P\left(\{S\},t\right)\right] \nonumber \\
    &= \sum_{\{S\}}S_{j}\left[W\left(-S_{j}\rightarrow S_{j}\right)P\left(\{S\}_{j},t\right) - W\left(S_{j}\rightarrow-S_{j}\right)P\left(\{S\},t\right)\right] \nonumber \\
   % &= \sum_{\{S\}}2S_{j}\left[-3 - S_{j-2}S_{j-1} - S_{j-1}S_{j+1} - S_{j+1}S_{j+2}+S_{j}\left(2S_{j-1}+2S_{j+1}+S_{j-2}+S_{j+2}\right)\right] \nonumber \\
    &= 2\left[2\left<S_{j-1}\right>+2\left<S_{j+1}\right>+\left<S_{j-2}\right>+\left<S_{j+2}\right>-3\left<S_{j}\right>\right] \nonumber \\
    &-2\left[\left<S_{j-2}S_{j-1}S_{j}\right>+\left<S_{j-1}S_{j}S_{j+1}\right>+\left<S_{j}S_{j+1}S_{j+2}\right>\right]. \label{meanmagchangeMR}
\end{align}
In order to derive equation (\ref{meanmagchangeMR}) we make use of the fact that $W\left(S_{k}\rightarrow -S_{k}\right) = W\left(-S_{k}\rightarrow S_{k}\right)$ and $\sum_{\{S\}}S_{j}P\left(\{S\}_{j}\right)=-\left<S_{j}\right>$. These respective symmetries and asymmetries result in the annihilation of all terms in the summation over $k$ with the exception of the $k=j$ term. For ease of notation we shall refer to $\left<S_{j}\left(t\right)\right>$ as $m_{1}$ from this point onwards, where $t$ dependence is implicit. Similarly, we shall refer to the three-point correlation function $\left<S_{j}\left(t\right)S_{j+1}\left(t\right)S_{j+2}\left(t\right)\right>$ as $m_{3}$. Using the fact that the system is spatially isotropic, we may write equation (\ref{meanmagchangeMR}) as
\begin{equation}\label{m1}
    \frac{dm_{1}}{dt} = 6\left(m_{1}-m_{3}\right).
\end{equation}
Equation (\ref{m1}) may look relatively innocent at first glance, though the hierarchical nature of correlation functions poses challenges. Just as the temporal evolution of $m_{1}$ is coupled to $m_{3}$, $m_{3}$ is coupled to even higher order correlation functions. As such, approximations are required in order to simplify the equations underlying the dynamics of the system. One approach to solving equation (\ref{m1}) would be to use the mean field approximation to factorise the three-point correlation function as $m_{3}=m_{1}^{3}$. The factorizability of correlation functions defines a mean field approximation in this context \cite{krapivsky2010kinetic}. However, a more sophisticated approach is adopted by the authors of \cite{mobilia2003majority} whereby the three-point correlation function is factorized as $m_{3}=m_{1}m_{2}$, where we define the two-point correlation function  $m_{2}=\left<S_{j}\left(t\right)S_{j+1}\left(t\right)\right>$.\newline

\noindent In order to proceed we must consider the degree to which the spins $S_{j}$ and $S_{j+r}$ are correlated, where $r\neq 0$. Let $W_{j} = W\left(S_{j}\rightarrow -S_{j}\right)$ and $W_{j+r} = W\left(S_{j+r}\rightarrow -S_{j+r}\right)$ be the spin flip rates at sites $j$ and $j+r$ respectively. Over the incremental time interval $\Delta t$, the quantity $S_{j}S_{j+r}$ changes as follows:
\begin{equation*}
    S_{j}\left(t+\Delta t\right)S_{j+r}\left(t+\Delta t \right) =
    \begin{cases}
    S_{j}\left(t\right)S_{j+r}\left(t\right)\quad \text{with probability}\quad 1-\left(W_{j}+W_{j+r}\right)\Delta t, \\
   - S_{j}\left(t\right)S_{j+r}\left(t\right)\quad \text{with probability}\quad\left(W_{j}+W_{j+r}\right)\Delta t.
    \end{cases}
\end{equation*} 
We can use this fact to express the temporal evolution of the quantity $\left<S_{j}\left(t\right)S_{j+r}\left(t\right)\right>$:
\begin{align}\label{SjSjr}
   &\frac{d}{dt}\left<S_{j}S_{j+r}\right> = -2\left<S_{j}S_{j+r}W\left(S_{j}\rightarrow -S_{j}\right)\right>-2\left<S_{j}S_{j+r}W\left(S_{j+r}\rightarrow -S_{j+r}\right)\right> \nonumber \\
   &= 2\left[\left<S_{j-2}S_{j+2}\right>+\left<S_{j+2}S_{j+r}\right>+2\left<S_{j-1}S_{j+r}\right>+2\left<S_{j+1}S_{j+r}\right>-6\left<S_{j}S_{j+r}\right>\right] \nonumber \\
   &+2\left[\left<S_{j}S_{j+r-2}\right>+\left<S_{j}S_{j+r+2}\right>+2\left<S_{j}S_{j+r-1}\right> + 2\left<S_{j}S_{j+r+1}\right>\right] \nonumber \\
   &-2\left[\left<S_{j-2}S_{j-1}S_{j}S_{j+r}\right>+ \left<S_{j-1}S_{j}S_{j+1}S_{j+r}\right>+\left<S_{j}S_{j+1}S_{j+2}S_{j+r}\right>\right] \nonumber \\
   &-\left[\left<S_{j}S_{j+r-2}S_{j+r-1}S_{j+r}\right>+\left<S_{j}S_{j+r-1}S_{j+r}S_{j+r+1}\right>+\left<S_{j}S_{j+r}S_{j+r+1}S_{j+r+2}\right>\right].
\end{align}
We adopt the notation used by Mobilia and Redner \cite{mobilia2003majority} in defining the following quantities: $c_{r}=\left<S_{j}\left(t\right)S_{j+|r|}\left(t\right)\right>$ and $m_{4} = \left<S_{j}\left(t\right)S_{j+1}\left(t\right)S_{j+2}\left(t\right)S_{j+3}\left(t\right)\right>$. It follows that $m_{2} = c_{1}=\left<S_{j}\left(t\right)S_{j\pm 1}\left(t\right)\right>$. This serves to simplify equation (\ref{SjSjr}). We proceed by implementing the Kirkwood approximation \cite{kirkwood1935statistical} to factorize the four-point correlation function as a product of two-point correlation functions: $m_{4} = m_{2}^{2}$. This approximation has proved successful in a number of other applications, ranging from the modelling of ecological population dynamics \cite{frachebourg1998fixation} to reaction kinetics \cite{schnorer1989segregation,lin1990joint}. Finally, we make the approximation that $c_{2}\approx c_{3}\approx m_{2}$ given that the spatial variation in the two-point correlation function is small as $t\rightarrow\infty$ \cite[Section 8.2]{krapivsky2010kinetic} and we are interested in studying the stationary distribution of the system. At this point our analysis diverges from the workings presented in \cite{mobilia2003majority} as there appears to be an algebraic error in the paper. Under these assumptions, equation (\ref{SjSjr}) simplifies as follows:
\begin{equation}\label{m2}
    \frac{dm_{2}}{dt} = -4\left(m_{2}+2\right)\left(m_{2}-1\right).
\end{equation}
It is straightforward to solve equation (\ref{m2}), with the final result being
\begin{equation}\label{m2answer}
    m_{2}\left(t\right) = \frac{1+2\beta e^{-12t}}{1-\beta e^{-12t}}\quad\text{where}\quad \beta=\frac{m_{2}\left(0\right)-1}{m_{2}\left(0\right)+2}.
\end{equation}
Equation (\ref{m2answer}) shows that $m_{2}\left(t\right)\rightarrow 1$ as $t\rightarrow\infty$. Using this result, we can proceed to solve equation (\ref{m1}) which can be rewritten as follows:
\begin{equation}\label{m1factorised}
    \frac{dm_{1}}{dt}=6m_{1}\left(1-m_{2}\right).
\end{equation}
Using equation (\ref{m2answer}) we can solve equation (\ref{m1factorised}) to give
\begin{equation}\label{m1answer}
    m_{1}\left(t\right) = m_{1}\left(0\right)\left(\frac{\beta-1}{\beta e^{-12t}-1}\right)^{3/2}.
\end{equation}
We determine the final magnetisation by looking at the limit of equation (\ref{m1answer}) as $t\rightarrow\infty$, in which case 
\begin{equation}\label{exitprob}
    m_{1}\left(\infty\right) = m_{1}\left(0\right)\left(1-\beta\right)^{3/2} = m_{1}\left(0\right)\left(\frac{3}{2+m_{1}\left(0\right)^{2}}\right)^{3/2}.
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth,height=8cm]{RingEP.eps}
    \caption[Exit probability on a ring of spins]{Simulation results on a ring of $N=100$ spins, with initial magnetisation plotted against final magnetisation. $10^{3}$ simulations were conducted for each value of $m_{1}\left(0\right)$.}
    \label{OneDimMagnetization}
\end{figure}

\noindent Equation (\ref{exitprob}) makes intuitive sense: if the population is initiated in a state of consensus then it will remain in that state for all time. Equation (\ref{exitprob}) differs from the exit probability $\mathcal{E}$ by a linear transformation: $\mathcal{E}=\left(m_{1}\left(\infty\right)+1\right)/2$. As such its qualitative interpretation is the same. Furthermore the final magnetisation is independent of the size of the system. In order to verify these findings numerically, simulations were conducted on a ring of $N=100$ spins. The results are displayed in Figure \ref{OneDimMagnetization} which illustrate that the analytical expression for $m_{1}\left(\infty\right)$ is in excellent agreement with the numerical simulations. The simulations were repeated on rings of different sizes though the results were the same, verifying that the final magnetisation is independent of $N$ in one dimension. Our analytical and numerical results are in notably better agreement than those presented in \cite{mobilia2003majority}. This concludes our study of MR dynamics on a ring.


==> abstract.tex <==
\begin{abstractlong}
The Majority Rule (MR) is used to model consensus formation in a population of interacting individuals or agents. Each agent in the population is assumed to be in one of a finite number of states. In a social context, the state of an individual could represent their opinion relating to a certain issue. In a physical context, this could correspond to the orientation of a magnetic dipole in a ferromagnetic material. The Majority Rule can be described as follows. At each update event, a subset of agents is chosen from the population to form an \textit{interaction group}. All agents in the group then simultaneously adopt the majority opinion in the group. This process is repeated \textit{ad infinitum} or until consensus is reached in the population. While the Majority Rule is simple in principle, in practice it gives rise to nontrivial dynamical behaviour. The associated dynamics are stochastic and highly nonlinear in nature. In addition, the multi-body nature of these interactions  may not be encoded in traditional graphical structures. In order to accurately model these dynamics we require a topological structure capable of encapsulating higher-order interactions. \textit{Hypergraphs} are ideal candidates in this regard. \newline

\noindent Throughout the course of this dissertation, we investigate MR dynamics on a wide range of hypergraph topologies. We restrict our attention to populations in which there are two competing opinions, which is representative of the presence of a polarising issue. We also restrict our attention to interaction groups of size $3$, or \textit{triangles}, which serves to simplify our analysis from a combinatorial perspective. We propose an original deterministic model to approximate MR dynamics on a broad range of hypergraph topologies. Our model proves to be an excellent predictor of the stochastic dynamics for large population sizes. In this sense, we aim to contribute to pre-existing knowledge in the field.
\end{abstractlong}

==> acknowledgements.tex <==
\begin{acknowledgements}
First, I would like to thank Prof. Renaud Lambiotte for his help and guidance over the past number of months. I have thoroughly enjoyed working on this project and exploring this area of mathematics. \newline

\noindent Secondly, I would like to thank Prof. Sidney Redner for his suggestions and constructive feedback. \newline

\noindent Finally, I would like to thank Dr Kathryn Gillow for her continued support and encouragement throughout the course of the MSc. It has been a stimulating programme of study and I have learned a tremendous amount.
\end{acknowledgements}
